A Case for Backward Compatibility for Human-AI Teams

AI systems are being deployed to support human decision making in high-stakes domains. In many cases, the human and AI form a team, in which the human makes decisions after reviewing the AI's inferences. A successful partnership requires that the human develops insights into the performance of the AI system, including its failures. We study the influence of updates to an AI system in this setting. While updates can increase the AI's predictive performance, they may also lead to changes that are at odds with the user's prior experiences and confidence in the AI's inferences, hurting therefore the overall team performance. We introduce the notion of the compatibility of an AI update with prior user experience and present methods for studying the role of compatibility in human-AI teams. Empirical results on three high-stakes domains show that current machine learning algorithms do not produce compatible updates. We propose a re-training objective to improve the compatibility of an update by penalizing new errors. The objective offers full leverage of the performance/compatibility tradeoff, enabling more compatible yet accurate updates.

==> ack.tex <==

\section{Acknowledgments}
% The authors would like to thank
% M. Ribeiro,
% S. Tan,
% X. Zhang,
% R. Caruana,
% M. Czerwinski,
% J. Suh,
% M. Joshi,
% J. Bragg,
% and anonymous reviewers for helpful feedback.
% Umar ??
% Adith Swaminathan
We thank  M.  Ribeiro,  S.  Tan,  X.
Zhang,  R.  Caruana,  M.  Czerwinski,  J.  Suh,  M.  Joshi,  J.
Bragg, and anonymous reviewers for helpful feedback. This work was
was supported by Microsoft Research, ONR grant N00014-18-1-2193, the future of Life foundation and the WRF/Cable Professorship.

==> content/old-text.tex <==
%%%%% from compatability.tex

% \Bug{Add paragraph to bridge gap between last and this definition of compatibility}
%Also, the developer may have access to other ``kinds'' of data, such as interaction history between users and $\hone$.
%In a previous section, we showed that an update is bad if it belongs to the no-intersection case.
%In other words, if $\htwo$ belongs to the no-intersection case, it may be a bad idea to deploy it.
%As a result, step 5 may be problematic.


% - A developer may update a classifier for many reasons
%     - collected additional training data
%     - new classification model or learning algorithm became available
% - We focus on the first reason: 
% - Typical ML pipeline:
%     - developer collects dtrainone
%     - trains hone on dtrainone and deploys it
%     - collects additional training data to create dtraintwo
%         - dtraintwo is a superset of dtrainone
%     - trains htwo on dtraintwo
%     - performance of htwo is higher than hone 
%     - developer deploys version 2

% - Notation:
%     - x: input
%     - y: true label
%     - hone: base classifier
%     - htwo: updated classifier
%     - htwocompat: compatible classifier 
%     - dtrainone: training set for hone
%     - dtraintwo: training set for htwo
%     - dtest: test set for hone and htwo


% Other :
% - dtraintwo=dtrainone, but htwo is different model class
% - interaction history between human and hone is available, learn htwo from both dtraintwo and interaction history.
%     - what if there are multiple interaction histories available?


%\Bug{WSL: Do we want to discuss the mental models that people form during the task a  little bit here? (This is the affinity diagramming over explanation)\\G: I think some qualitative example of mental model would be useful. Not sure if we should put one from study or make up something or pick up something from the internet.}

%\Bug{WSL: I would break this next part into a new section}

